Fairness for Image Generation with Uncertain Sensitive Attributes

This work tackles the issue of fairness in the context of generative procedures, such as image super-resolution, which entail different definitions from the standard classification setting. Moreover, while traditional group fairness definitions are typically defined with respect to specified protected groups -- camouflaging the fact that these groupings are artificial and carry historical and political motivations -- we emphasize that there are no ground truth identities. For instance, should South and East Asians be viewed as a single group or separate groups? Should we consider one race as a whole or further split by gender? Choosing which groups are valid and who belongs in them is an impossible dilemma and being "fair" with respect to Asians may require being "unfair" with respect to South Asians. This motivates the introduction of definitions that allow algorithms to be \emph{oblivious} to the relevant groupings. We define several intuitive notions of group fairness and study their incompatibilities and trade-offs. We show that the natural extension of demographic parity is strongly dependent on the grouping, and \emph{impossible} to achieve obliviously. On the other hand, the conceptually new definition we introduce, Conditional Proportional Representation, can be achieved obliviously through Posterior Sampling. Our experiments validate our theoretical results and achieve fair image reconstruction using state-of-the-art generative models.

==> table-cat80dog20.tex <==
\begin{figure*}[h]
	\begin{subtable}[t]{0.48\linewidth}
		\vspace{-13em}
		\centering
		\resizebox{\columnwidth}{!}{%
		\begin{tabular}[scale=0.9]{|c|c|c|c|c|}
			\hline 
			\multirow{2}{*}{$m$} & \multicolumn{2}{|c|}{PULSE} &
			\multicolumn{2}{|c|}{Ours} \\
			\cline{2-5}
			& Cats & Dogs & Cats &
			Dogs \\
			\hline
			$1\times 1$  & 0 & 125 & 115 & 96 \\
			$2\times 2$  & 0 & 125 & 82 & 97 \\
			$4\times 4$  & 0 & 125 & 94 & 86 \\
			$8\times 8$  & 1 & 123 & 71 & 94 \\
			\hline
		\end{tabular}
		}
		\caption{\small Number of errors on 80\% cat generator, for each
		resolution. Sampled test set has \textbf{500} cats and
		\textbf{125} dogs from the AFHQ validation set to mimick the
		generator's training distribution.  PULSE makes errors on almost
		all the dogs and no cats, while Posterior Sampling is
		relatively balanced.}
	\end{subtable}
	\begin{subfigure}[t]{0.48\linewidth}
		\centering
		\includegraphics[scale=0.35]{figures/error_bar_binomial_cat80dog20-2867.pdf}
		\caption{\small Fraction of all errors on cats for 80\% cat generator.}
	\end{subfigure}
  \caption{\small Same as in Figure~\ref{fig:cat20dog80}, except now we use a
  StyleGAN2 trained on 80\% cats. Again, PULSE is clearly biased
towards the majority, whiel Posterior Sampling via Langevin dynamics
appears to satisfy SPE.}
	% \caption{We use a StyleGAN2 model trained on 80\% cats and report
	% errors when reconstructing images from low-resolution measurements. 
    	% The test set consists of 
	% 500 cats and 125 dogs from the AFHQ validation set to mimick
	% the generator's training distribution (note that these correspond to
	% all cats in the AFHQ validation set).  Figure (b) shows the
	% proportion of all errors that are on cats, along with 95\%
	% confidence intervals from a binomial test. An algorithm that
	% satisfies SPE would have this probability=0.5 (green line). PULSE is
	% clearly biased towards the majority, while Posterior Sampling 
	% via Langevin dynamics appears to satisfy SPE.  }
	\label{fig:cat80dog20}
\end{figure*}


==> theory.tex <==
\section{Notation}

We use:
\begin{enumerate}
	\item $R:$ data distribution.
	\item $P:$ generator's distribution.
	\item $\pi( y | x):$ conditional distribution of measurements
		$y$ given signal $x$.
	\item $\varphi(y) = \int_{x \in \R^n} r(x) \pi(y|x) dx,$ is the
		distribution induced over $y$ if the source distribution is $r$.
	\item $\psi(y) = \int_{x \in \R^n} p(x) \pi(y|x) dx,$ is the
		distribution induced over $y$ if the source distribution is $p$.
\end{enumerate}

\section{Case 1: $P=R$}

\begin{claim}
	Assume $P=R$. For any two sets $U \& V \subset \R^n,$ we have
	\begin{align*}
		\Pr_{x^* \sim P, y \sim \pi( \cdot | x^*) , \wh{x} \sim P( \cdot |
		y)}\left[ x^* \in U, \wh{x} \in V \right] &= \Pr_{x^* \sim P, y
		\sim \pi( \cdot | x^*) , \wh{x} \sim P( \cdot | y)}\left[ x^* \in
		V, \wh{x} \in U \right]
	\end{align*}
\end{claim}

\begin{proof}
	We have
	\begin{align*}
		\Pr_{x^* \sim P, y \sim \pi( \cdot | x^*) , \wh{x} \sim P( \cdot |
		y)}\left[ x^* \in U, \wh{x} \in V \right] 
		&= \int_{x^* \in U, \wh{x} \in V} p(x^*) \pi(y | x^*) p(\wh{x} |
		y) dx^* dy d\wh{x},\\
		&= \int_{x^* \in U, \wh{x} \in V} p(x^*) \pi(y | x^*)
		\frac{\pi(y | \wh{x}) p(\wh{x})}{\psi(y)} dx^* dy d\wh{x},\\
		&= \int_{x^* \in V, \wh{x} \in U} p(x^*) \pi(y | x^*)
		\frac{\pi(y | \wh{x}) p(\wh{x})}{\psi(y)} dx^* dy d\wh{x},\\
		&= \Pr_{x^* \sim P, y \sim \pi( \cdot | x^*) , \wh{x} \sim P( \cdot |
		y)}\left[ x^* \in V, \wh{x} \in U \right]
	\end{align*}
\end{proof}


\section{Case 2: $TV(P,R) \leq \delta$}

\begin{claim}
	Assume that $TV(R,P) \leq \delta.$ For any two sets $U \& V \subset
	\R^n,$ we have
	\begin{align*}
		\Pr_{x^* \sim R, y \sim \pi( \cdot | x^*) , \wh{x} \sim P( \cdot |
		y)}\left[ x^* \in U, \wh{x} \in V \right] &= \Pr_{x^* \sim P, y
		\sim \pi( \cdot | x^*) , \wh{x} \sim P( \cdot | y)}\left[ x^* \in
		V, \wh{x} \in U \right] \pm 2 \delta.
	\end{align*}
\end{claim}

\begin{proof}
	Let 
	$$q = \Pr_{x^* \sim P, y \sim \pi( \cdot | x^*) , \wh{x} \sim P(
	\cdot | y)}\left[ x^* \in U, \wh{x} \in V \right] $$

	From Claim ?? we have 
	$$q = \Pr_{x^* \sim P, y \sim \pi( \cdot | x^*) , \wh{x} \sim P(
	\cdot | y)}\left[ x^* \in V, \wh{x} \in U \right].$$

	We have
	\begin{align}
		\Pr_{x^* \sim R, y \sim \pi( \cdot | x^*) , \wh{x} \sim P( \cdot |
		y)}\left[ x^* \in U, \wh{x} \in V \right] 
		&= \int_{x^* \in U, \wh{x} \in V} r(x^*) \pi(y | x^*) p(\wh{x} |
		y) dx^* dy d\wh{x},\nonumber\\
		&= \int_{x^* \in U, \wh{x} \in V} p(x^*)  \pi(y | x^*)
		\frac{\pi(y | \wh{x}) p(\wh{x})}{\psi(y)} dx^* dy d\wh{x} ,\nonumber\\
		& + \int_{x^* \in U, \wh{x} \in V} \left( r(x^*) -  p(x^*)  \right)\pi(y | x^*)
		\frac{\pi(y | \wh{x}) p(\wh{x})}{\psi(y)} dx^* dy d\wh{x} \nonumber\\
		&= q + \int_{x^* \in U} \left( r(x^*) - p(x^*)  \right)\Pr_{y \sim
		\pi(\cdot | x^*), \wh{x} \sim P(\cdot | y)}\left[ \wh{x} \in V
		\right] dx^* .\label{eqn:claim2eqn1}
	\end{align}

	Consider the term 
	$$\int_{x^* \in U} \left( r(x^*) - p(x^*)  \right)\Pr_{y \sim
	\pi(\cdot | x^*), \wh{x} \sim P(\cdot | y)}\left[ \wh{x} \in V
	\right].  $$

	Since $TV(R, P) \leq \delta,$ we have 
	\begin{align*}
		\int_{x^* \in U} (r(x^*) - p(x^*)) \Pr\left[ \wh{x} \in V | x^*
		\right]
		&\leq \int_{x^* \in U, r(x^*) > p(x^*)} (r(x^*) - p(x^*)) \Pr\left[ \wh{x} \in V | x^*
		\right],\\
		& \leq \int_{x^* \in \R^n, r(x^*) > p(x^*)} r(x^*) - p(x^*))
		\Pr\left[ \wh{x} \in V | x^* \right],\\
		& \leq \int_{x^* \in \R^n, r(x^*) > p(x^*)} r(x^*) - p(x^*)),\\
		&= TV(R,P) \leq \delta.
	\end{align*}

	A similar proof gives
	\begin{align*}
		\int_{x^* \in U} (r(x^*) - p(x^*)) \Pr\left[ \wh{x} \in V | x^*
		\right] \geq - \delta.
	\end{align*}

	Substituting in Eqn~\eqref{eqn:claim2eqn1}, we have
	\begin{align*}
		\Pr_{x^* \sim R, y \sim \pi( \cdot | x^*) , \wh{x} \sim P( \cdot |
		y)}\left[ x^* \in U, \wh{x} \in V \right] = q \pm \delta.
	\end{align*}

	By symmetry, we can consider the event $x^* \in V, \wh{x} \in U,$ we
	have
	\begin{align*}
		\Pr_{x^* \sim R, y \sim \pi( \cdot | x^*) , \wh{x} \sim P( \cdot |
		y)}\left[ x^* \in V, \wh{x} \in U \right] = q \pm \delta.
	\end{align*}

	The above two inequalities prove the claim.


\end{proof}

\section{Case 3: $W_\infty(R,P) \leq \varepsilon$}

We make the following assumptions:
\begin{enumerate}
	\item $W_\infty(R,P) \leq \varepsilon.$
		\ajil{Make a stronger assumption on 1 so that we can get a weaker
		assumption for 2.}
	\item Let $\Gamma$ be the optimal coupling between $R\& P.$ Let
		$(x^*, x) \sim \Gamma,$ and by the $W_\infty$ assumption, we have
		$\norm{x^* - x} \leq \varepsilon$ almost surely. Then the
		measurement distribution satisfies:
		\begin{align}
			\norm{\pi( \cdot | x^*) - \pi( \cdot | x)}_{TV} \leq \delta.
		\end{align}
	\item The sets $U$ \& $V$ satisfy
		\begin{align*}
			\max\left\{ R( U \oplus B_{2\varepsilon} \setminus U), R( V
			\oplus
			B_{2\varepsilon} \setminus V), P( U \oplus B_{\varepsilon} \setminus
			U), P( V \oplus B_{\varepsilon} \setminus V) \right\} \leq \delta.
		\end{align*}
		where $B_{\varepsilon}$ denotes the $\ell_2-$ball with radius
		$\varepsilon$ and $\oplus$ denotes the Minkowski sum between the
		two sets.
\end{enumerate}


\subsection{Discussion}
When is assumption 2 satisfied?
If $\pi( y | x) = \cN(Ax, \sigma^2 I)$, then we have
\begin{align*}
	\norm{ \pi( \cdot | x) - \pi(\cdot | x^*) }_{TV} \leq 4.5
	\frac{\norm{Ax - Ax^*}_2}{\sigma}
\end{align*}
If $A : \R^n \to \R^{m}$ blurs pixels in blocks of size
$\frac{n}{m},$ then we have

\begin{align*}
	\norm{ \pi( \cdot | x) - \pi(\cdot | x^*) }_{TV} \leq 4.5
	\frac{\varepsilon}{\sigma \sqrt{\frac{n}{m}}}
\end{align*}

Hence if $\sigma \gtrsim \frac{\varepsilon}{\delta
\sqrt{\frac{n}{m}}},$ then Assumption 2 is satisfied.  Note that this
measurement process effectively destroys information between $x \&
x^*$ that are $\varepsilon-$close. 

Alternatively, we could consider the setting of our previous paper,
where $$\pi(y | x) = \cN(Ax, \frac{\sigma^2}{m} I_m),$$ and $A$ is
Gaussian i.i.d. In this setting, $U \& V$ are sets of radius $r
\geq \varepsilon$, separated by $\geq C r$ for some large enough
constant $C$. In this case, our previous results imply that $$\Pr\left[
x^* \in U, \wh{x} \in V \right] \approx \Pr\left[ x^* \in V, \wh{x}
\in U \right] \leq e^{-\Omega(m)}$$. In this measurement process,
information is \emph{preserved} between sets that are sufficiently
separated.

\subsection{Lemma and Proof}
\begin{lemma}\label{lemma:winf}
	Under the above assumptions, if $x^* \sim R, y \sim \pi( \cdot |
	x^*),$ and $\wh{x}\sim P( \cdot | y),$ then we have

	\begin{align*}
		\Pr_{x^*, y , \wh{x}}\left[ x^* \in U, \wh{x} \in V \right] &=
		\Pr_{x^*, y , \wh{x}}\left[ x^* \in V, \wh{x} \in U \right] \pm 4
		\delta.
	\end{align*}


\end{lemma}

\begin{proof}
	
	Let $\Gamma$ denote the optimal $\cW_\infty$ coupling between $R \&
	P.$

	Let $q_{uv}$ denote the probability that $x^* \in U$ and $\wh{x} \in
	V$ when $x^*$ is drawn according to $R$. Similarly, let $p_{uv}$
	denote the same event when $x^*$ is drawn according to $P.$  Then we
	have
	\begin{align}
		q_{uv}:=\Pr_{x^*, y , \wh{x}}\left[ x^* \in U, \wh{x} \in V \right] &=
		\int_{x^* \in U, x , y, \wh{x} \in V} \gamma( x^*, x) \pi(y| x^*)
		p( \wh{x} | y) dx^* dx dy d\wh{x},\nonumber\\
		&= \int_{x^* \in U, x , y, \wh{x} \in V} \gamma( x^*, x) (\pi(y|
		x^*) - \pi( y|x) ) p(\wh{x}|y) dx^* dx dy d\wh{x}(*) \\
		&+ \int_{x^* \in U, x , y, \wh{x} \in V} \gamma( x^*, x) \pi(y| x)
		p(\wh{x}|y) dx^* dx dy d\wh{x}. (**)
	\end{align}

	From Claim~\ref{claim:winf-pi}, we have
	\begin{align}
		-\delta \leq (*) \leq \delta.
	\end{align}

	From Claim~\ref{claim:winf-gamma}, we have
	\begin{align*}
		p_{uv} - \min\left\{ R\left( U \oplus B_{2\varepsilon} \setminus U
		\right), P\left( U \oplus B_{\varepsilon} \right) \right\} \leq (**) \leq p_{uv} + P\left[ U \oplus B_{\varepsilon} \setminus U
		\right].
	\end{align*}

	From the assumptions on $U$, we have
	\begin{align*}
		p_{uv} - 2\delta \leq q_{uv} \leq p_{uv} + 2\delta.
	\end{align*}

	A symmetric proof gives us
	\begin{align*}
		p_{vu} - 2\delta \leq q_{vu} \leq p_{vu} + 2\delta.
	\end{align*}

	Using the above two inequalities, and the fact that $p_{vu} =
	p_{uv},$ we have
	\begin{align*}
		-4	\delta \leq q_{uv} - q_{vu} \leq 4 \delta.
	\end{align*}

\end{proof}

\begin{claim}\label{claim:winf-pi}
	Consider the term $(*)$ in Lemma~\ref{lemma:winf}. We have 
	$$ -\delta \leq (*) \leq \delta.$$
\end{claim}
\begin{proof}
	Consider the term $(*)$. We have 
	\begin{align}
		(*) &= \int_{x^* \in U, x , y, \wh{x} \in V} \gamma( x^*, x)
		(\pi(y| x^*) - \pi( y|x) ) p(\wh{x} |y) dx^* dx dy,\\
		&= \int_{x^* \in U, x , y} \gamma( x^*, x) (\pi(y| x^*) - \pi(
		y|x) ) \Pr(\wh{x} \in V |y) dx^* dx dy,\\
		&\leq \int_{x^* \in U, x , y: \pi(y | x^*) \geq \pi(y | x) }
		\gamma( x^*, x) (\pi(y| x^*) - \pi( y|x) ) \Pr(\wh{x} \in V |y)
		dx^* dx dy,\\
		&\leq \int_{x^* \in U, x , y: \pi(y | x^*) \geq \pi(y | x) }
		\gamma( x^*, x) (\pi(y| x^*) - \pi( y|x) ) ,\\
		&= \int_{x^* \in U, x } \gamma( x^*, x) \norm{\pi( \cdot | x^*) -
		\pi( \cdot | x) }_{TV},\\
		&\leq \int_{x^* \in U, x } \gamma( x^*, x) \delta \leq \delta.
	\end{align}
	where the last line follows from the assumptions.

	A similar proof gives
	\begin{align}
		(*) \geq - \delta.
	\end{align}
	
	This gives us $$ - \delta \leq (*) \leq \delta.$$
	
\end{proof}

\begin{claim}\label{claim:winf-gamma}
	Consider the term $(**)$ in Lemma~\ref{lemma:winf}. We have
	\begin{align*}
		p_{uv} - \min\left\{ R\left( U \oplus B_{2\varepsilon} \setminus U
		\right), P\left( U \oplus B_{\varepsilon} \right) \right\} \leq (**) \leq p_{uv} + P\left[ U \oplus B_{\varepsilon} \setminus U
		\right].
	\end{align*}
\end{claim}

\begin{proof}
	We have
	\begin{align}
		(**) & = \int_{x^* \in U, x , y, \wh{x} \in V} \gamma( x^*, x)
		\pi(y| x) p(\wh{x}|y) ,\\
		&= \int_{x^* \in U, x \in U \oplus B_\varepsilon} \int_{ y, \wh{x}
		\in V} \gamma( x^*, x) \pi(y| x) p(\wh{x}|y) ,\\
		&= \int_{x^* \in U \oplus B_{2\varepsilon}, x \in U \oplus
		B_\varepsilon} \int_{ y, \wh{x} \in V} \gamma( x^*, x) \pi(y| x)
		p(\wh{x}|y) (\dagger)\\
		&- \int_{x^* \in U \oplus B_{2\varepsilon} \setminus U, x \in U \oplus
		B_\varepsilon} \int_{ y, \wh{x} \in V} \gamma( x^*, x) \pi(y| x)
		p(\wh{x}|y) , (\dagger\dagger).
	\end{align}

	It is easy to see that 
	$$ 0 \leq (\dagger\dagger) \leq \min\left\{ R(U \oplus B_{2\varepsilon},
	P(U + B_{\varepsilon}) \right\}.$$

	In order to bound $(\dagger)$, notice that the only term with $x^*$
	is $\gamma$. Further, by the $W_\infty$ assumption, we have
	$\int_{x^* \in U \oplus B_{2\varepsilon}, x \in U \oplus
	B_{\varepsilon}} \gamma(x^*, x)= \int_{x\in U \oplus
	B_{\varepsilon}} p(x).$

	This gives
	\begin{align}
		(\dagger) &= \int_{x \in U \oplus B_{\varepsilon}} p(x)
		\int_{y , \wh{x} \in V} \pi(y | x) p(\wh{x} | y),\\
		&= \int_{x \in U } p(x) \int_{y , \wh{x} \in V} \pi(y | x)
		p(\wh{x} | y) + \int_{x \in U \oplus B_{\varepsilon} \setminus U}
		p(x) \int_{y , \wh{x} \in V} \pi(y | x) p(\wh{x} | y),\\
	\end{align}

	This gives 
	$$ p_{uv} \leq \left( \dagger  \right)\leq p_{uv} + P( U \oplus
	B_{\varepsilon} \setminus U) .$$


	The above bounds give
	\begin{align*}
		p_{uv} - \min\left\{ R\left( U \oplus B_{2\varepsilon} \setminus U
		\right), P\left( U \oplus B_{\varepsilon} \right) \right\} \leq (**) \leq p_{uv} + P\left[ U \oplus B_{\varepsilon} \setminus U
		\right].
	\end{align*}
	
\end{proof}


\section{Case 4: $\cW_\infty(R,P) \leq \varepsilon$}

We make the following assumptions on the distributions:
\begin{enumerate}
	\item For $\class \in \left\{ \cat, \dog \right\},$ we have
	
		$$ -\delta \leq P(\class) - R(\class) \leq \delta.$$

	\item For $\class \in \left\{ \cat, \dog \right\},$ the conditional
		distributions satisfy 
		$$\cW_{\infty, \delta}(R(\cdot | \class), P(\cdot | \class ))\leq
		\varepsilon.$$

	\item For $x^*, x$ such that $\norm{x^* -x } \leq \varepsilon,$ the
		measurement distribution satisfies:
		\begin{align}
			\norm{\pi( \cdot | x^*) - \pi( \cdot | x)}_{TV} \leq \delta,
		\end{align*}
		almost surely over $x^*, x.$
\end{enumerate}

\begin{lemma}
	Under the assumptions of the above lemma, we have
	\label{lemma:winfdelta}
\end{lemma}


\begin{proof}
	Let $q_12$ denote the probability of a cat being reconstructed as a
	dog, when $x^*$ is drawn from $R$.

	Then we have
	\begin{align*}
		q_{12} &= \int_{x^* \in \cat, \wh{x} \in \dog} r(x^*) \pi(y | x^*)
		p(\wh{x} | y) ,\\
		&= R(x^* \in \cat) \int_{\wh{x} \in \dog} r(x^* | x^* \in \cat)
		\pi(y | x^*) p(\wh{x} | y),\\
		&= P(x^* \in \cat) \int_{\wh{x} \in \dog} r(x^* | x^* \in \cat)
		\pi(y | x^*) p(\wh{x} | y) \pm \delta,\\
		&= P(x^* \in \cat) (1-c_1) \int_{\wh{x} \in \dog} r'(x^* | x^* \in
		\cat) \pi(y | x^*) p(\wh{x} | y) (*)\\
		&+ P(x^* \in \cat) c_1 \int_{\wh{x} \in \dog} r''(x^* | x^* \in
		\cat) \pi(y | x^*) p(\wh{x} | y) (**),\\
		& \pm \delta.
	\end{align*}
	By the $\cW_{\infty,\delta}$ condition, we have that $c_1 \leq
	\delta$. This gives 
	$$(**) \leq \delta.$$

	Now we consider term $(*)$. We have
	\begin{align*}
		(*) &= P(x^* \in \cat) (1-c_1) \int_{\wh{x} \in \dog} r'(x^* | x^*
		\in \cat) \pi(y | x^*) p(\wh{x} | y) \\
		&= P(x^* \in \cat) (1-c_1) \int_{\wh{x} \in \dog} \gamma (x^*, x | x^* \in \cat, x
		\in \cat) \pi(y | x^*) p(\wh{x} | y) \\
		&= P(x^* \in \cat) (1-c_1) \int_{\wh{x} \in \dog} \gamma (x^*, x | x^* \in \cat, x
		\in \cat) \pi(y | x) p(\wh{x} | y) (\dagger)\\
		&+ P(x^* \in \cat) (1-c_1) \int_{\wh{x} \in \dog} \gamma (x^*, x | x^* \in \cat, x
		\in \cat) (\pi(y | x^*) - \pi(y|x))p(\wh{x} | y) (\dagger\dagger) \\
	\end{align*}

	From Claim ??, we have 
	\begin{align*}
		- \delta \leq (\dagger \dagger) \leq \delta.
	\end{align*}

	Now for $(\dagger),$ and since $\gamma$ is a coupling between $r' \&
	p',$ we have
	\begin{align*}
		(\dagger) &= P(x^* \in \cat) (1-c_1) \int_{\wh{x} \in \dog} p' (x | x \in \cat) \pi(y | x) p(\wh{x} | y) \\
		&= P(\cat) (1-c_1) \int_{\wh{x} \in \dog} p' (x | x \in
		\cat) \pi(y | x) \frac{\pi(y | \wh{x}) p(\wh{x})}{\psi(y)} \\
		&= P(\cat) (1-c_1) \int_{\wh{x} \in \dog} p' (x | x \in \cat)
		\pi(y | x) \frac{\pi(y | \wh{x}) P(\dog) ( (1-c_2)p'(\wh{x} |
		\wh{x} \in \dog) + c_2 p''(\wh{x}| \wh{x} \in \dog))}{\psi(y)} \\
	\end{align*}

	\ajil{The term involving $p'$ is nice because it is symmetric for
	$x^* \in \cat$ and $x^* \in \dog$. How do I handle the term with
	$p''$? I think we may need to consider the sets $ \supp(P'(\cdot |
	\cat)) \& \supp(P'(\cdot | \dog)).$}



\end{proof}

